Local Causal Discovery for Structural Evidence of Direct Discrimination

Identifying the causal pathways of unfairness is a critical objective for improving policy design and algorithmic decision-making. Prior work in causal fairness analysis often requires knowledge of the causal graph, hindering practical applications in complex or low-knowledge domains. Moreover, global discovery methods that learn causal structure from data can display unstable performance on finite samples, preventing robust fairness conclusions. To mitigate these challenges, we introduce local discovery for direct discrimination (LD3): a method that uncovers structural evidence of direct unfairness by identifying the causal parents of an outcome variable. LD3 performs a linear number of conditional independence tests relative to variable set size, and allows for latent confounding under the sufficient condition that all parents of the outcome are observed. We show that LD3 returns a valid adjustment set (VAS) under a new graphical criterion for the weighted controlled direct effect, a qualitative indicator of direct discrimination. LD3 limits unnecessary adjustment, providing interpretable VAS for assessing unfairness. We use LD3 to analyze causal fairness in two complex decision systems: criminal recidivism prediction and liver transplant allocation. LD3 was more time-efficient and returned more plausible results on real-world data than baselines, which took 46$\times$ to 5870$\times$ longer to execute.

==> figure_tex/compas/compas.tex <==
\begin{figure}
    \centering
\input{figure_tex/compas/compas_05_ds} \\ \vspace{10mm}
\input{figure_tex/compas/compas_05_ty} 
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

==> figure_tex/figure_flow.tex <==
\begin{figure}
    \centering

\tikzstyle{terminator} = [rectangle, draw, text centered, rounded corners, minimum height=2em]
\tikzstyle{process} = [rectangle, draw, text centered, minimum height=2em]
\tikzstyle{decision} = [diamond, draw, text centered, minimum height=2em]
\tikzstyle{outline} = [rectangle,draw,dotted,thick]
\tikzstyle{data}=[trapezium, draw, text centered, trapezium left angle=60, trapezium right angle=120, minimum height=2em]
\tikzstyle{connector} = [draw, -{Latex[width=4pt]}, thick]

\begin{tikzpicture}
\node [process, fill=Blue!20, draw=Blue] at (-3.5,2)  (scm) {\footnotesize\textit{SCM}};
\node [process, fill=Blue!20, draw=Blue] at (-3.5,0)(true) {\footnotesize\textit{True graph}};
\node [outline,Blue,text depth=3cm, minimum height=3cm, minimum width=2cm] at (-3.55,1.25) (dgp) {\footnotesize\textsc{DGP}};

 \node [process, fill=Maroon!20, draw=Maroon] at (-0.5,2) (data) {\footnotesize\textit{Observed data}};
\node [process, fill=Maroon!20, draw=Maroon] at (-0.5,1) (disc) {\footnotesize\textit{Discovery method}};
\node [process, fill=Maroon!20, draw=Maroon] at (-0.5,0) (learned) {\footnotesize\textit{Learned graph}};
\node [outline,Maroon,text depth=3cm, minimum height=3cm] at (-0.5,1.25) (dgp) {\footnotesize\textsc{Causal Discovery}};

\node [process, fill=MidnightBlue!20, draw=MidnightBlue] at (3,2) (crit) {\footnotesize\textit{Structural criteria}};
\node [process, fill=MidnightBlue!20, draw=MidnightBlue] at (3,0) (emp) {\footnotesize\textit{Empirical estimates}};
\node [outline,MidnightBlue,text depth=3cm, minimum height=3cm] at (3,1.25) (dgp) {\footnotesize\textsc{Fairness Analysis}};

\path [connector,Blue] (scm) -- (data);
\path [connector,Blue] (scm) -- (true);
\path [connector,Maroon] (data) -- (disc);
\path [connector,Maroon] (disc) -- (learned);
\path [connector,Maroon] (data) -- (emp);
\path [connector,Maroon] (learned) -- (emp);
%\path [connector,gray!60] (true) -- (fair);
%\path [connector,gray!60] (true) -- (crit);
%\path [connector] (error) |- (end);

% Declare these here so that (data) -- (emp) arrow goes behind fair box.
\node [process, fill=MidnightBlue!20, draw=MidnightBlue] at (3,1) (fair) {\footnotesize\textit{Fairness measures}};
\path [connector,MidnightBlue] (crit) -- (fair);
\path [connector,MidnightBlue] (fair) -- (emp);


\end{tikzpicture}


    \caption{An expanded map of the causal fairness analysis framework, where access to the true causal graph is not assumed. Instead, global or local structure is learned from observational data. 
    From left to right: (1) the true data generating process (DGP) is defined by the structural causal model (SCM), which dictates the ground truth causal graphical structure; (2) causal discovery recovers the causal graph from data sampled from the DGP; (3) causal fairness analysis defines criteria and measures based on the causal structure, and empirical estimates are obtained using knowledge from the learned graph. Adapted from \citet{plecko_causal_2024} (Figure 1.3).}
    \label{fig:flow}
\end{figure}

==> figure_tex/figure_full_graph.tex <==
\begin{figure}
\begin{adjustbox}{max width=\textwidth}
\centering
\fbox{\input{figure_tex/figure_step_1}}
%%%%%%%%
\hspace{2mm}
%%%%%%%%
\fbox{\input{figure_tex/figure_step_2}}
%%%%%%%%
\hspace{2mm}
%%%%%%%%
\fbox{\input{figure_tex/figure_step_3}}
%%%%%%%%
\hspace{2mm}
%%%%%%%%
\fbox{\input{figure_tex/figure_ld3_graph}}
\end{adjustbox}
    \caption{The local subgraph identified by LD3. In this setting,  $\z_1$, $\z_3$, and $\z_4$ are members of these partitions that are directly adjacent to $Y$.}
    \label{fig:full_graph}
\end{figure}

==> figure_tex/figure_true_to_sfm.tex <==
\begin{figure}[!h]
    \centering
    \input{figure_tex/figure_projection}
    \caption{Causal fairness discovery is concerned with learning the projection of the true graph $\mathcal{G}$ (left) onto the Standard Fairnes Model (SFM; right). $\mathcal{G}$ can be reduced to a ten node DAG (left), where each node represents a set corresponding to a causal partition with respect to protected attribute $X$ and outcome $Y$ \citep{maasch2024local}. To assess  causal fairness, we then project $\mathcal{G}$ onto the SFM to obtain $\g_{SFM}$ \citep{plecko_causal_2024}. In the outcome control setting, $D$ represents a decision that is known to influence $Y$ \citep{plecko_causal_2023}. In this projection, we abstract away all nodes except those pertinent to causal fairness analysis: decision $D \in \z_1 \cup \z_4 \cup \z_3$, set $\mathbf{C} \subseteq \z_1$ (i.e., confounders), and $\mathbf{M} \subseteq \z_3$ (i.e., mediators). All edges signify paths of length $\geq 1$. Gray dotted edges are unknown \textit{a priori} and must be discovered from data, while black edges represent prior knowledge (e.g., from domain expertise).}
    \label{fig:projection}
\end{figure}


==> figure_tex/liver/liver.tex <==
\begin{figure}
    \centering
\input{figure_tex/liver/ld3_17-19_01} \hspace{8mm}
\input{figure_tex/liver/pc_17-19_01} \hspace{8mm}
\input{figure_tex/liver/ldecc_17-19_01} \\
\vspace{10mm}
\input{figure_tex/liver/ld3_20-22_01} \hspace{8mm}
\input{figure_tex/liver/pc_20-22_01} \hspace{8mm}
\input{figure_tex/liver/ldecc_20-22_01}
    \caption{Predicted parent sets, SDC, and WCDE estimates for STAR liver data. Exposure is patient sex (\textit{S}; {\color{WildStrawberry}red}) and outcome is receiving a liver (\textit{L}; {\color{CornflowerBlue}blue}). Known parents of $L$ are in {\color{Dandelion}yellow}. \textit{AE} = active exception case; \textit{BT} = recipient blood type; \textit{DX} = diagnosis; \textit{ED} = education; \textit{ET} = ethnicity; \textit{EX} = exception type; \textit{IA} = initial age; \textit{IM} = initial MELD; \textit{PM} = payment method; \textit{RE} = region; \textit{WE} = weight. WCDE is reported with $p$-value ($p$) and 95\% confidence intervals in brackets. All methods used $\chi^2$ independence tests ($\alpha = 0.01$).}
    \label{fig:liver_all_results}
\end{figure}

==> tables/table_andes.tex <==
\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l c c c c c}
    \toprule
        & \multicolumn{5}{c}{\textbf{\textsc{Andes}}} \\
        \cmidrule(lr){2-6}
        & \textit{F1} & \textit{Prec} & \textit{Rec} & \textit{Time} & \textit{Tests} \\
        \midrule
        LD3 & 0.94 [0.88,1.00] & 0.92 [0.84,1.00] & 0.98 [0.93,1.00] & 0.71 [0.669,0.75] & 557.3 [549.66,564.94] \\
        LDECC$_\cup$ \\
        LDP$_{pa}$ & 0.18 [0.1,0.27] & 0.11 [0.06,0.17] & 0.52 [0.27,0.78] & 0.367 [0.359,0.375] & 580.1 [570.56,589.64] \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


==> tables/table_bnlearn.tex <==
\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l l c c c c c c}
    \toprule
    & & \multicolumn{6}{c}{\textsc{\textbf{Asia (Lung Cancer)}}} \\
    \cmidrule(lr){3-8}
    %%%
    & & \multicolumn{2}{c}{SDC = 1: either $\to$ dysp} & \multicolumn{2}{c}{SDC = 0: xray $\to$ dysp} \\
    \cmidrule(lr){3-5}  \cmidrule(lr){6-8}
    %%%%
    & & \textit{F1} & \textit{Prec} & \textit{Rec} & \textit{F1} & \textit{Prec} & \textit{Rec} \\
    %%%%
    \midrule
    \parbox[t]{1cm}{\multirow{4}{*}{\textit{Oracle}}}
    & LD3  &  &  &  &  &  &  \\
    & PC$_\cup$  &  &  &  &  &  &  \\
    & PC$_\cap$  &  &  &  &  &  &  \\
    & LDECC$_\cup$  &  &  &  &  &  &  \\
    & LDECC$_\cap$  &  &  &  &  &  &  \\
    & LDP$_{pa}$  &  &  &  &  &  &  \\
    & LDP &  &  &  &  &  &  \\
    %%%%
    \midrule
    \parbox[t]{1cm}{\multirow{4}{*}{$n = 5k$}}
    & LD3  &  &  &  &  &  &  \\
    & PC$_\cup$  &  &  &  &  &  &  \\
    & PC$_\cap$  &  &  &  &  &  &  \\
    & LDECC$_\cup$  &  &  &  &  &  &  \\
    & LDECC$_\cap$  &  &  &  &  &  &  \\
    & LDP$_{pa}$  &  &  &  &  &  &  \\
    & LDP &  &  &  &  &  &  \\
    %%%%
    \midrule
    \parbox[t]{1cm}{\multirow{4}{*}{$n = 10k$}}
    & LD3  &  &  &  &  &  &  \\
    & PC$_\cup$  &  &  &  &  &  &  \\
    & PC$_\cap$  &  &  &  &  &  &  \\
    & LDECC$_\cup$  &  &  &  &  &  &  \\
    & LDECC$_\cap$  &  &  &  &  &  &  \\
    & LDP$_{pa}$  &  &  &  &  &  &  \\
    & LDP &  &  &  &  &  &  \\
    %%%%
    \midrule
    \parbox[t]{1cm}{\multirow{4}{*}{$n = 20k$}}
    & LD3  &  &  &  &  &  &  \\
    & PC$_\cup$  &  &  &  &  &  &  \\
    & PC$_\cap$  &  &  &  &  &  &  \\
    & LDECC$_\cup$  &  &  &  &  &  &  \\
    & LDECC$_\cap$  &  &  &  &  &  &  \\
    & LDP$_{pa}$  &  &  &  &  &  &  \\
    & LDP &  &  &  &  &  &  \\
    %%%%
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Empirical performance on Sachs protein network data from \texttt{bnlearn} with chi-square independence tests ($\alpha = 0.001$; 95\% confidence intervals in brackets).}
    \label{tab:asia}
\end{table}

%&  &  &  &  &  &  \\

% To rotate multirow:
%\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{$n = 10k$}}}

\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l l c c c c}
    \toprule
    & & \multicolumn{4}{c}{\textsc{\textbf{Asia (Lung Cancer)}}} \\
    \cmidrule(lr){3-6}
    %%%
    & & \multicolumn{2}{c}{SDC = 1: either $\to$ dysp} & \multicolumn{2}{c}{SDC = 0: xray $\to$ dysp} \\
    \cmidrule(lr){3-4}  \cmidrule(lr){5-6}
    %%%%
    & & \textit{Time} & \textit{Tests} & \textit{Time} & \textit{Tests} \\
    %%%%
    \midrule
    \parbox[t]{1cm}{\multirow{4}{*}{\textit{Oracle}}}  & LD3 &  &  &  &  \\
    & PC &  &  &  &  \\
    & LDECC &  &  &  &  \\
    & LDP &  &  &  &  \\
    %%%%
    \midrule
    \parbox[t]{1cm}{\multirow{4}{*}{$n = 5k$}}  & LD3 &  &  &  &  \\
    & PC &  &  &  &  \\
    & LDECC &  &  &  &  \\
    & LDP &  &  &  &  \\
    %%%%
    \midrule
    \parbox[t]{1cm}{\multirow{4}{*}{$n = 10k$}}  & LD3 &  &  &  &  \\
    & PC &  &  &  &  \\
    & LDECC &  &  &  &  \\
    & LDP &  &  &  &  \\
    %%%%
    \midrule
    \parbox[t]{1cm}{\multirow{4}{*}{$n = 20k$}}  & LD3 &  &  &  &  \\
    & PC &  &  &  &  \\
    & LDECC &  &  &  &  \\
    & LDP &  &  &  &  \\
    %%%%
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Total number of independence tests performance and runtimes in seconds.}
    \label{tab:asia_time_tests}
\end{table}

==> tables/table_liver_time.tex <==
\begin{table}[!h]
    \centering
    \begin{adjustbox}{max width=0.5\textwidth}
    \begin{tabular}{c c c c c c c c}
    \toprule
    %%
       & & \multicolumn{2}{c}{\textsc{\textbf{LD3}}}  & \multicolumn{2}{c}{\textsc{\textbf{PC}}} & \multicolumn{2}{c}{\textsc{\textbf{Ratio PC/LD3}}} \\
       \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
       %%
       \textit{Policy} & $\alpha$ & \textit{Time} & \textit{Tests} & \textit{Time} & \textit{Tests} & \textit{Time} & \textit{Tests} \\
       \midrule
       %%
       \parbox[t]{1.5cm}{\multirow{2}{*}{2017-2019}} & 0.01 & \textbf{0.100} & \textbf{75} & 237.324 & 35943 & 2373.24 & 479.24 \\
       & 0.05 & \textbf{0.101} & \textbf{75} & 231.844 & 36512 & 2295.48 & 486.83 \\
       %%
       \midrule
       %%
       \parbox[t]{1.5cm}{\multirow{2}{*}{2020-2022}} & 0.01 & \textbf{0.107} & \textbf{75} & 465.278 & 63225 & 4348.39 & 843.00 \\
       & 0.05 & \textbf{0.090} & \textbf{71} & 528.372  & 72517 & 5870.80 & 1021.37 \\
    \bottomrule
    \end{tabular} \\
    \end{adjustbox}
    \vspace{3mm}
    \caption{Total number of independence tests performance and runtimes in seconds for LD3 vs PC Algorithm on the liver transplant allocation dataset \citep{kalisch_estimating_2007}.}
    \label{tab:ld3_pc_time_tests}
\end{table}
